Privacy Preserving Set-Based Estimation Using Partially Homomorphic Encryption

The set-based estimation has gained a lot of attention due to its ability to guarantee state enclosures for safety-critical systems. However, collecting measurements from distributed sensors often requires outsourcing the set-based operations to an aggregator node, raising many privacy concerns. To address this problem, we present set-based estimation protocols using partially homomorphic encryption that preserve the privacy of the measurements and sets bounding the estimates. We consider a linear discrete-time dynamical system with bounded modeling and measurement uncertainties. Sets are represented by zonotopes and constrained zonotopes as they can compactly represent high-dimensional sets and are closed under linear maps and Minkowski addition. By selectively encrypting parameters of the set representations, we establish the notion of encrypted sets and intersect sets in the encrypted domain, which enables guaranteed state estimation while ensuring privacy. In particular, we show that our protocols achieve computational privacy using the cryptographic notion of computational indistinguishability. We demonstrate the efficiency of our approach by localizing a real mobile quadcopter using ultra-wideband wireless devices.

==> figures/prt1.tex <==
%% Creator: Inkscape inkscape 0.92.4, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'prt1.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{276.24599309bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.79711199)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{figures/prt1.pdf}}%
    \put(0.04216116,0.02371831){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Sensor Node S1\end{tabular}}}}%
    \put(0.69048537,0.02343036){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Sensor Node S2\end{tabular}}}}%
    \put(0.39130821,0.41502652){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Aggregator A\end{tabular}}}}%
    \put(0.31489112,0.72991768){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Intersection\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{figures/prt1.pdf}}%
    \put(0.07905217,0.25296957){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Strips\end{tabular}}}}%
    \put(0.71410443,0.14883772){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Strips\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{figures/prt1.pdf}}%
  \end{picture}%
\endgroup%


==> figures/prt1_old.tex <==
%% Creator: Inkscape inkscape 0.92.5, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'pri_set.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{276.24655151bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  
  \def\scale{0.9}
  
  \begin{picture}(0.9,0.79811558)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\scale\unitlength,page=1]{figures/prt1.pdf}}%
    \put(0.42315235,0.13327765){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\Huge...\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\scale\unitlength,page=2]{figures/prt1.pdf}}%
    \put(0.35579336,0.41768265){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Aggregator $\mathbb{A}$\end{tabular}}}}%
    \put(0.04425878,0.01){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Sensor Node $\mathbb{S}_1$\end{tabular}}}}%
    \put(0.62231721,0.01){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Sensor Node $\mathbb{S}_{m_a}$\end{tabular}}}}%
    \put(0.31596451,0.71588724){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Intersection\end{tabular}}}}%
    \put(0.05592895,0.19515658){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Strips\end{tabular}}}}%
    \put(0.65,0.19515658){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Strips\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> figures/prt1_oold.tex <==
%% Creator: Inkscape inkscape 0.92.5, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'prt1.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{276.2460022bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.79710933)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{figures/prt1.pdf}}%
    \put(0.04216115,0.02371564){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Sensor Node $\mathbb{S}_1$\end{tabular}}}}%
    \put(0.69048534,0.0234277){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Sensor Node $\mathbb{S}_2$\end{tabular}}}}%
    \put(0.3913082,0.41502384){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Aggregator $\mathbb{A}$\end{tabular}}}}%
    \put(0.31489111,0.72991499){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Intersection\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{figures/prt1.pdf}}%
    \put(0.07905216,0.25296689){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Strips\end{tabular}}}}%
    \put(0.72632178,0.2479315){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Strips\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> figures/prt1_tex_oo.tex <==
%% Creator: Inkscape inkscape 0.92.5, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'prt1.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{276.2460022bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  

  \begin{picture}(1,0.79710933)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{figures/prt1.pdf}}%
    \put(0.33197744,0.72603195){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Intersection\end{tabular}}}}%
    \put(0.46782726,0.17183655){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}{$\cdots$}\end{tabular}}}}%
    \put(0.390883054,0.41114819){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Aggregator $\mathbb{A}$\end{tabular}}}}%
    \put(0.06515748,0.02249164){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Sensor Node $\mathbb{S}_1$\end{tabular}}}}%
    \put(0.70520271,0.01889305){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Sensor Node $\mathbb{S}_{m}$\end{tabular}}}}%
    \put(0.07017409,0.23931164){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Strips\end{tabular}}}}%
    \put(0.71772762,0.23931164){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Strips\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> figures/prt2.tex <==
%% Creator: Inkscape inkscape 0.92.4, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'prt2.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{428.65975186bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.78149013)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{figures/prt2.pdf}}%
    \put(0.11258539,0.00422374){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Sensor Group G1\end{tabular}}}}%
    \put(0.68505081,0.00523283){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Sensor Group G2\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{figures/prt2.pdf}}%
    \put(0.31770671,0.74729223){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Diffusion\end{tabular}}}}%
    \put(0.42886925,0.46078408){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Aggregator A\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{figures/prt2.pdf}}%
  \end{picture}%
\endgroup%


==> figures/prt2_oold.tex <==
%% Creator: Inkscape inkscape 0.92.5, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'prt2.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{430.62854004bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.79697438)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{figures/prt2.pdf}}%
    \put(0.09060623,0){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Sensor Group $\mathbb{G}^{(1)}$\end{tabular}}}}%
    \put(0.6444544,0){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Sensor Group $\mathbb{G}^{(2)}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{figures/prt2.pdf}}%
    \put(0.31878975,0.75943095){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Diffusion\end{tabular}}}}%
    \put(0.41044407,0.46423269){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Aggregator $\mathbb{A}$\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> figures/prt2_tex_oo.tex <==
%% Creator: Inkscape inkscape 0.92.5, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'prt2.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{430.62854004bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  
  \begin{picture}(0.55,0.45697438)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{figures/prt2.pdf}}%
    \put(0.16469083,0.41008704){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Diffusion\end{tabular}}}}%
    \put(0.05034395,0.01990415){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Sensor Group $\mathbb{G}_1$\end{tabular}}}}%
    \put(0.21,0.25){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Aggregator $\mathbb{A}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{figures/prt2.pdf}}%
    \put(0.3504395,0.01990415){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Sensor Group $\mathbb{G}_{m}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{figures/prt2.pdf}}%
    %\put(0.02249867,0.15455384){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}strips\end{tabular}}}}%
    %\put(0.27296975,0.15455384){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}strips\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{figures/prt2.pdf}}%
    %\put(0.05154923,0.29884525){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}intersection\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{figures/prt2.pdf}}%
    \put(0.11,0.07){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}…\end{tabular}}}}%
    %\put(0.57610804,0.15455384){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}strips\end{tabular}}}}%
    %\put(0.8265559,0.15455384){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}strips\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=6]{figures/prt2.pdf}}%
    %\put(0.60518182,0.29884525){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}intersection\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=7]{figures/prt2.pdf}}%
    \put(0.26,0.11){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}…\end{tabular}}}}%
    \put(0.42,0.07){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}…\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> figures/results/CZS_esterr_data.tex <==
\addplot [black]
  table[row sep=crcr]{%
1	0.333212684969762\\
6	0.598671245514094\\
11	0.618527447540222\\
16	0.594712213256947\\
21	0.455166601308124\\
26	0.425008564002402\\
31	0.405285793405132\\
36	0.41843666448866\\
41	0.433017243393896\\
46	0.411714347048744\\
51	0.309710059480577\\
56	0.213132927909048\\
61	0.152666824237696\\
66	0.0943518471343068\\
71	0.104915055222487\\
76	0.109391622013002\\
81	0.0883684440559166\\
86	0.0744617173001993\\
91	0.0783236167114482\\
96	0.0640205809560648\\
101	0.0670329315839763\\
106	0.0810726398955872\\
111	0.0797406468411315\\
116	0.0769688023651248\\
121	0.0696590020075196\\
126	0.0669211072471472\\
131	0.0601036639873901\\
136	0.0730632308418693\\
141	0.135517859533667\\
146	0.168788514111905\\
151	0.134939231758159\\
156	0.10528573474521\\
161	0.125333507892224\\
166	0.195808992264186\\
171	0.221202136524699\\
176	0.195327308915591\\
181	0.182908254300538\\
186	0.174201866273745\\
191	0.200835061087896\\
196	0.22517021592607\\
201	0.217538703706856\\
206	0.166195664068836\\
211	0.123458088821415\\
216	0.126520395834875\\
221	0.122983585090192\\
226	0.169629831348628\\
231	0.233956442039864\\
236	0.25380680361939\\
241	0.258346456648298\\
246	0.251538438681473\\
251	0.255506217492245\\
256	0.265296998923448\\
261	0.233473323387149\\
266	0.201716521490453\\
271	0.209421767524268\\
276	0.244197336904027\\
281	0.265554310746274\\
286	0.268987883875611\\
291	0.273359811937476\\
296	0.270288896233231\\
301	0.29554795877959\\
306	0.320573470121132\\
311	0.318987046623825\\
316	0.273551343058204\\
321	0.22700831218948\\
326	0.223424287195094\\
331	0.20329400562961\\
336	0.189131651122514\\
341	0.19162377927965\\
346	0.191018569672487\\
351	0.192827028134218\\
356	0.192580963164684\\
361	0.22056437863148\\
366	0.248162505067169\\
371	0.212679053382909\\
376	0.156030858777142\\
381	0.124089254868153\\
386	0.132486865736063\\
391	0.152438076194743\\
396	0.154693780992334\\
401	0.155890371515846\\
406	0.156792626107512\\
411	0.137555104780174\\
416	0.119039898718793\\
421	0.120477002764691\\
426	0.126069436962422\\
431	0.127665605236239\\
436	0.182979451562924\\
441	0.243725247241213\\
446	0.247862788981349\\
451	0.254908337810144\\
456	0.262995010754142\\
461	0.262458018059395\\
466	0.201488551755249\\
471	0.148352912388956\\
476	0.163764641602324\\
481	0.176472122248459\\
486	0.191626004307341\\
491	0.174967813206632\\
496	0.117664815095649\\
501	0.103151382973701\\
506	0.0922202589349514\\
511	0.0962434805727043\\
516	0.118932577966622\\
521	0.122383179254825\\
526	0.133418484772071\\
531	0.145236718417414\\
536	0.15503871705615\\
541	0.161225048110603\\
546	0.203512461492348\\
551	0.242407345932478\\
556	0.192929674685096\\
561	0.14658630455282\\
566	0.135198750820717\\
571	0.114903207352703\\
576	0.117872442774831\\
581	0.12699136223915\\
586	0.128981304716718\\
591	0.135791497924055\\
596	0.136273213705602\\
601	0.136747324303417\\
606	0.145662127257463\\
611	0.145843910630557\\
616	0.145292356077807\\
621	0.168485022412396\\
626	0.218336794820387\\
631	0.274275313568022\\
636	0.268771918519886\\
641	0.200912660782376\\
646	0.180489129907441\\
651	0.19565936021081\\
656	0.21160075197439\\
661	0.227362525163446\\
666	0.202886024866619\\
671	0.180103992107794\\
676	0.193443457449234\\
681	0.211337718670594\\
686	0.204761416898552\\
691	0.199509201011838\\
696	0.170089860191398\\
701	0.125132585254833\\
706	0.115295043257737\\
711	0.121380821196129\\
716	0.117510911430191\\
721	0.111053835684707\\
726	0.124872867290042\\
731	0.139667409264175\\
736	0.138794236468776\\
741	0.143121920640994\\
746	0.191638377354898\\
751	0.2205511036289\\
756	0.221869270971693\\
761	0.252799138959013\\
766	0.302401444068354\\
771	0.353905005269556\\
776	0.448616291901292\\
781	0.452861714655719\\
786	0.376417417165885\\
791	0.371590135112295\\
796	0.338178214026099\\
801	0.298438880326462\\
806	0.298228897193856\\
811	0.272854131665765\\
816	0.257528767179197\\
821	0.268253144164356\\
826	0.218157977859151\\
831	0.16588161827076\\
836	0.169914292879406\\
841	0.159305957080113\\
846	0.171905496280318\\
851	0.208560080830236\\
856	0.215878548122415\\
861	0.225739141313255\\
866	0.25061714305254\\
871	0.273460299405212\\
876	0.303381867195065\\
881	0.332095475389449\\
886	0.360841235271087\\
891	0.377903966687824\\
896	0.375051479011255\\
901	0.376359634968419\\
906	0.372182897044681\\
911	0.370270291464577\\
916	0.367932253372697\\
921	0.34002196099248\\
926	0.326665297302543\\
931	0.336256493209567\\
936	0.336776729978821\\
941	0.344928732730315\\
946	0.355145490034316\\
951	0.350351456470224\\
956	0.35457323583833\\
961	0.368177143694864\\
966	0.377605674286857\\
971	0.385551507555763\\
976	0.392702164015621\\
981	0.386656131167346\\
986	0.368240421889201\\
991	0.370052473055234\\
996	0.381807824730719\\
1001	0.353233937728777\\
1006	0.333115901603891\\
1011	0.348299017232925\\
1016	0.322377369520177\\
1021	0.281272434327866\\
1026	0.274166878968099\\
1031	0.26008386522585\\
1036	0.248479573145947\\
1041	0.235921061815359\\
1046	0.209159291512542\\
1051	0.208591835021482\\
1056	0.218625040723862\\
1061	0.208767076907128\\
1066	0.196080355144535\\
1071	0.215836055040921\\
1076	0.218798185046644\\
1081	0.215395660819042\\
1086	0.226859316528793\\
1091	0.212193835777649\\
1096	0.198544936720584\\
1101	0.213909829083347\\
1106	0.231140768600233\\
1111	0.207176701322437\\
1116	0.177850697273546\\
1121	0.181840022273526\\
1126	0.190854181577189\\
1131	0.176323612134008\\
1136	0.172471902644916\\
1141	0.189711149871911\\
1146	0.172945732021385\\
1151	0.156191117286083\\
1156	0.170812831677201\\
1161	0.178076826461145\\
1166	0.170455279828773\\
1171	0.182556702348469\\
1176	0.209751576786785\\
1181	0.203161310382757\\
1186	0.178408819337268\\
1191	0.171055413855099\\
1196	0.162386833279541\\
1201	0.149851900450079\\
1206	0.174827018304423\\
1211	0.201029948542964\\
1216	0.177049217185351\\
1221	0.154826848722879\\
1226	0.155669895948426\\
1231	0.158576722086252\\
1236	0.146032900532077\\
1241	0.142349539066368\\
1246	0.155380358782243\\
1251	0.158570580703898\\
1256	0.153312120539319\\
1261	0.14431678334144\\
1266	0.147412800512348\\
1271	0.15706352332125\\
1276	0.150366628086053\\
1281	0.147698085208257\\
1286	0.1577161655777\\
1291	0.166639177411782\\
1296	0.158308100108855\\
1301	0.150788408422613\\
1306	0.173145824314151\\
1311	0.192529321023662\\
1316	0.197582324831929\\
1321	0.211891635530092\\
1326	0.231881443407666\\
1331	0.220285961872021\\
1336	0.19004453402167\\
1341	0.186019410319503\\
1346	0.207818699148908\\
1351	0.191528040722741\\
1356	0.171636765937153\\
1361	0.212039493136953\\
1366	0.242448968570226\\
1371	0.209741700234412\\
1376	0.190997243994596\\
1381	0.200441321973442\\
1386	0.201178888040692\\
1391	0.197779475534711\\
1396	0.183660271059742\\
1401	0.192641885309118\\
1406	0.209067466411949\\
1411	0.196471949380811\\
1416	0.179818182622415\\
1421	0.184070921585692\\
1426	0.178809647386517\\
1431	0.150275970044934\\
1436	0.133209315212199\\
1441	0.15033200070913\\
1446	0.16124469568296\\
1451	0.145117959054481\\
1456	0.134574350189357\\
1461	0.133898816849584\\
1466	0.13392419540605\\
1471	0.12355621033738\\
1476	0.102280707435141\\
1481	0.102988800880092\\
1486	0.11264691047801\\
1491	0.12146316303629\\
1496	0.121533891672925\\
1501	0.111252518065017\\
1506	0.116403067465726\\
1511	0.111679291215718\\
1516	0.0988354128583133\\
1521	0.112006617734598\\
1526	0.125401486020346\\
1531	0.110954116579846\\
1536	0.109700062658234\\
1541	0.115717472680474\\
1546	0.113779511145019\\
1551	0.112888763947255\\
1556	0.10836938786013\\
1561	0.119359473010215\\
1566	0.144219297290973\\
1571	0.145450614150738\\
1576	0.133440485364582\\
1581	0.133137888154058\\
1586	0.130059638280822\\
1591	0.109860282490462\\
1596	0.0978042624782252\\
1601	0.0993620194755861\\
1606	0.106636503782068\\
1611	0.116696708253323\\
1616	0.0947980874262978\\
1621	0.0781730868349162\\
1626	0.0841534016813911\\
1631	0.0844184786856449\\
1636	0.0993259180370669\\
1641	0.102680417062217\\
1646	0.0899975236644992\\
1651	0.0949112341204609\\
1656	0.102757566476606\\
1661	0.105398624911355\\
1666	0.105556086253266\\
1671	0.107286879410006\\
1676	0.107964251717405\\
1681	0.113846924200572\\
1686	0.110632387109121\\
1691	0.101643684585483\\
1696	0.108443038527627\\
1701	0.128484599715531\\
1706	0.13042960199958\\
1711	0.123553160677568\\
1716	0.129563781413712\\
1721	0.135562384056308\\
1726	0.154018093946041\\
1731	0.135132382364136\\
1736	0.104994187743466\\
1741	0.111368377299806\\
1746	0.117161643527053\\
1751	0.112205960578279\\
1756	0.104168505310403\\
1761	0.103550125765492\\
1766	0.106707693186841\\
1771	0.0931951791004079\\
1776	0.0784268013850482\\
1781	0.0808117985709804\\
1786	0.109942766935148\\
1791	0.138653356097344\\
1796	0.130852695504106\\
1801	0.129647072479751\\
1806	0.136048807557431\\
1811	0.145708178286306\\
1816	0.160737731503388\\
1821	0.148993850260064\\
1826	0.126917762575079\\
1831	0.139671232674953\\
1836	0.165991469904\\
1841	0.169074635830018\\
1846	0.152979537963154\\
1851	0.145137589456714\\
1856	0.154234774513692\\
1861	0.168184400551604\\
1866	0.172277119813156\\
1871	0.159404886171201\\
1876	0.154433756971077\\
1881	0.157326682145343\\
1886	0.158257618420697\\
1891	0.167632340241788\\
1896	0.153080370488997\\
1901	0.130546284956089\\
1906	0.133912116145779\\
1911	0.130026326812646\\
1916	0.122297652852428\\
1921	0.145108481306329\\
1926	0.166477668398965\\
1931	0.159609672665617\\
1936	0.15129732608148\\
1941	0.148586619085451\\
1946	0.149714736528887\\
1951	0.162723768552954\\
1956	0.175231899964926\\
1961	0.173735347878648\\
1966	0.171085689983066\\
1971	0.169705195594828\\
1976	0.153108111444809\\
1981	0.137423281797751\\
1986	0.129763492829268\\
1991	0.125422862957906\\
1996	0.122551516686154\\
2001	0.118345180614474\\
2006	0.115601250777004\\
2011	0.121321024468126\\
2016	0.132163415272546\\
2021	0.123761823691643\\
2026	0.107355742631901\\
2031	0.103454714000625\\
2036	0.107763452752185\\
2041	0.107139727771711\\
2046	0.101791465049765\\
2051	0.0811535761248745\\
2056	0.0792623216972042\\
2061	0.0956099681149375\\
2066	0.1071714308358\\
2071	0.127562163020029\\
2076	0.130451795008511\\
2081	0.120129565853842\\
2086	0.128993542911361\\
2091	0.124699376589692\\
2096	0.110650841640237\\
2101	0.125569649852229\\
2106	0.141879432930681\\
2111	0.143506945084482\\
2116	0.137604804715525\\
2121	0.133074227474227\\
2126	0.133545745413443\\
2131	0.138586814351395\\
2136	0.163381263621621\\
2141	0.17550009401538\\
2146	0.171964096975906\\
2151	0.177902130877415\\
2156	0.168883571731406\\
2161	0.160127535118957\\
2166	0.149798417201609\\
2171	0.140047830013179\\
2176	0.144141091952692\\
2181	0.163693363969139\\
2186	0.170575540234429\\
2191	0.161324492467601\\
2196	0.150585377513309\\
2201	0.14243829003852\\
2206	0.153375627420625\\
2211	0.156996452882398\\
2216	0.155682736380957\\
2221	0.144482184198618\\
2226	0.142215884529493\\
2231	0.15015744006201\\
2236	0.154660130754683\\
2241	0.153230156041485\\
2246	0.152627531774435\\
2251	0.138200346704823\\
2256	0.115100764989389\\
2261	0.117285663343495\\
2266	0.131204193947235\\
2271	0.127754080732572\\
2276	0.115172017595459\\
2281	0.135578583240307\\
2286	0.150275397549494\\
2291	0.137574636500094\\
2296	0.1241849631854\\
2301	0.116872573393534\\
2306	0.115770245809507\\
2311	0.113893701727403\\
2316	0.126321224891757\\
2321	0.129691485539604\\
2326	0.126654137745986\\
2331	0.137054300978789\\
2336	0.141549788219985\\
2341	0.140239406723943\\
2346	0.116606307627366\\
2351	0.0980082202318918\\
2356	0.0959984061761729\\
2361	0.107907250265353\\
2366	0.11745994831803\\
2371	0.112871461554756\\
2376	0.134738404594639\\
2381	0.150694566794614\\
2386	0.146126314522931\\
2391	0.146965883481433\\
2396	0.142354480246423\\
2401	0.145536051128809\\
2406	0.155973970314192\\
2411	0.153610185546619\\
2416	0.153352964823581\\
2421	0.158042668753119\\
2426	0.164093306999712\\
2431	0.145479149504791\\
2436	0.120575962281681\\
2441	0.118593682668815\\
2446	0.106935698564736\\
2451	0.113619991306152\\
2456	0.119806204870922\\
2461	0.129580671495525\\
2466	0.148067880615865\\
2471	0.132492559906064\\
2476	0.117218803669358\\
2481	0.114174303601116\\
2486	0.11307116262428\\
2491	0.123052941715073\\
2496	0.147403223909259\\
2501	0.147162171758833\\
2506	0.14174184744089\\
2511	0.150676287032334\\
2516	0.151546305739478\\
2521	0.15622302807395\\
2526	0.146281149507422\\
2531	0.134637334725987\\
2536	0.13609293388758\\
2541	0.136146486630289\\
2546	0.13465909752297\\
2551	0.154194748603381\\
2556	0.173992920082957\\
2561	0.171969129119944\\
2566	0.170804175627827\\
2571	0.171036680013623\\
2576	0.171199310530248\\
2581	0.192154713095366\\
2586	0.207757467832215\\
2591	0.199079006220162\\
2596	0.195950906244958\\
2601	0.190354803373604\\
2606	0.20073403156919\\
2611	0.204649189786917\\
2616	0.1938237447003\\
2621	0.195083877003862\\
2626	0.212835679236751\\
2631	0.222163332968059\\
2636	0.2140862394131\\
2641	0.237535551378337\\
2646	0.265844069142973\\
2651	0.260856278321948\\
2656	0.247086548412256\\
2661	0.238870019725407\\
2666	0.235317307436407\\
2671	0.242023852224816\\
2676	0.248412387945754\\
2681	0.244918327368493\\
2686	0.248465471050696\\
2691	0.261070757220484\\
2696	0.26868134494867\\
2701	0.265167700297416\\
2706	0.25886928248484\\
2711	0.258871835375158\\
2716	0.272323448188253\\
2721	0.264381184859951\\
2726	0.241844058734946\\
2731	0.255011911248837\\
2736	0.281142524062396\\
2741	0.289734139577863\\
2746	0.274977587108001\\
2751	0.254539075324967\\
2756	0.24499902467464\\
2761	0.269353241375884\\
2766	0.27968917678447\\
2771	0.267131544356716\\
2776	0.267922096114194\\
2781	0.291323023338746\\
2786	0.317752462344333\\
2791	0.314305546745536\\
2796	0.307353627019983\\
2801	0.299535053331938\\
2806	0.286523097349037\\
2811	0.281061964816333\\
2816	0.30197861801179\\
2821	0.323955566094755\\
2826	0.30458329904275\\
2831	0.278392550332502\\
2836	0.274892961483144\\
2841	0.27128225447917\\
2846	0.265164790147235\\
2851	0.274198498313775\\
2856	0.271012298792518\\
2861	0.265841297178469\\
2866	0.274941108024526\\
2871	0.285745701247642\\
2876	0.284524964107206\\
2881	0.272626272369173\\
2886	0.272873862273558\\
2891	0.272669122448991\\
2896	0.272178922508909\\
2901	0.273652768066682\\
2906	0.289348446458693\\
2911	0.308141615851678\\
2916	0.303200720233107\\
2921	0.297022872141642\\
2926	0.289891844466067\\
2931	0.278811002400538\\
2936	0.277832951338114\\
2941	0.264972265619265\\
2946	0.258205143807934\\
2951	0.263567114916692\\
2956	0.270598071645443\\
2961	0.268095093807455\\
2966	0.258047551944931\\
2971	0.258169159408653\\
2976	0.298554492108807\\
2981	0.335543309072667\\
2986	0.332977496010515\\
2991	0.350078373687766\\
2996	0.394163668060714\\
3001	0.41264683145957\\
3006	0.400833527548181\\
3011	0.387171347156717\\
3016	0.377151546886538\\
3021	0.417480578761663\\
3026	0.442620524231551\\
3031	0.446645316909195\\
3036	0.468303525354779\\
3041	0.506732093175182\\
3046	0.520354145693898\\
3051	0.504748069518174\\
3056	0.511866723165711\\
3061	0.482860594550845\\
3066	0.417483480827823\\
3071	0.383587989133426\\
3076	0.392415053853054\\
3081	0.401220853665976\\
3086	0.364709780801877\\
3091	0.300038897330944\\
3096	0.272635127429138\\
3101	0.258340858295005\\
3106	0.230406046393955\\
3111	0.208055076559442\\
3116	0.190284989161867\\
3121	0.174044712123777\\
3126	0.167446422649274\\
3131	0.174235194091979\\
3136	0.185533085083931\\
3141	0.187134657232158\\
3146	0.249710363682813\\
3151	0.324850350262437\\
3156	0.333965579987838\\
3161	0.349494279345392\\
3166	0.363966121244404\\
3171	0.404991965760967\\
3176	0.434148530975189\\
3181	0.419186889299345\\
3186	0.403374283324487\\
3191	0.388249879545906\\
3196	0.430221661626017\\
3201	0.471418632858233\\
3206	0.466336862796336\\
3211	0.461691765114232\\
3216	0.459302645966536\\
3221	0.458251706215426\\
3226	0.460694070547326\\
3231	0.464545200370265\\
3236	0.467477996027745\\
3241	0.466994040036316\\
3246	0.46538798426675\\
3251	0.47720664322186\\
3256	0.497034103190422\\
3261	0.501440752842293\\
3266	0.489301715421656\\
3271	0.473290234936257\\
3276	0.469431178435194\\
3281	0.477681980603236\\
3286	0.48734998882754\\
3291	0.484178765319853\\
3296	0.483972283446519\\
3301	0.503864004492607\\
3306	0.486367238783207\\
3311	0.457227564800967\\
3316	0.4568699058075\\
3321	0.428592122572517\\
3326	0.36286988148896\\
3331	0.322566967392314\\
3336	0.32387631438689\\
3341	0.330391515238167\\
3346	0.318267452596998\\
3351	0.286645602980093\\
3356	0.269233214038207\\
3361	0.271468474244375\\
3366	0.279853141667694\\
3371	0.300022044341964\\
3376	0.321985301438408\\
3381	0.332997860350945\\
3386	0.362397490079096\\
3391	0.387859118868959\\
3396	0.387619698171684\\
3401	0.388343813528237\\
3406	0.40502432497054\\
3411	0.443857971996794\\
3416	0.468166910721856\\
3421	0.479910970310437\\
3426	0.554427801829731\\
3431	0.611636632992496\\
3436	0.596315479344798\\
3441	0.588874883365339\\
3446	0.678449406494571\\
3451	0.752233698333183\\
3456	0.72419444718078\\
3461	0.711541878791471\\
3466	0.703211153057881\\
3471	0.689910006223437\\
3476	0.681392616180847\\
3481	0.676689543869787\\
3486	0.739958436659465\\
3491	0.795941101369735\\
3496	0.788144852111458\\
3501	0.789113110294107\\
3506	0.82946738688202\\
3511	0.866114868988116\\
3516	0.849061756340974\\
3521	0.83321214360775\\
3526	0.782711932366269\\
3531	0.732273391792086\\
3536	0.726001298153326\\
3541	0.721457247334584\\
3546	0.721686989606004\\
3551	0.722093842329806\\
3556	0.722067019102941\\
3561	0.721349727510264\\
3566	0.709797910855123\\
3571	0.721907596286081\\
3576	0.741510668997042\\
3581	0.737827840013262\\
3586	0.781837965010381\\
};

==> figures/results/ZS_esterr_data.tex <==
\addplot [black]
  table[row sep=crcr]{%
1	0.332135614093623\\
6	0.601502479219278\\
11	0.56755140667993\\
16	0.559696994509078\\
21	0.461564894455071\\
26	0.409204610439693\\
31	0.39736925085265\\
36	0.397488352224896\\
41	0.418805906999339\\
46	0.414892277725052\\
51	0.355434831455182\\
56	0.268224741270512\\
61	0.164647480720598\\
66	0.0927982869545772\\
71	0.102562696614246\\
76	0.109118601929146\\
81	0.091331786320395\\
86	0.073148726022317\\
91	0.073402376044197\\
96	0.0659254417872549\\
101	0.0623358042776267\\
106	0.0728841894189332\\
111	0.0771892214057784\\
116	0.0671809332220277\\
121	0.0577363217915634\\
126	0.0636387827156674\\
131	0.0626796959832359\\
136	0.0732908473288493\\
141	0.123230653650545\\
146	0.158698405649987\\
151	0.149462524539104\\
156	0.124824545491587\\
161	0.0954464591076859\\
166	0.115163069012468\\
171	0.171832211510956\\
176	0.195779677367256\\
181	0.192299399990982\\
186	0.181803234051549\\
191	0.192558025491532\\
196	0.215433223058037\\
201	0.220013127631528\\
206	0.191230834796319\\
211	0.153891360877206\\
216	0.136523955573613\\
221	0.12677591592436\\
226	0.141786106828264\\
231	0.19695935687477\\
236	0.239318555381023\\
241	0.252280304906881\\
246	0.255473143558734\\
251	0.259661836837649\\
256	0.267165530040856\\
261	0.252210819474085\\
266	0.223838466671592\\
271	0.210742569739088\\
276	0.236111830007839\\
281	0.262437266759759\\
286	0.269219457150494\\
291	0.27624841133047\\
296	0.276443801580867\\
301	0.2958316979576\\
306	0.318873458131501\\
311	0.320635829665366\\
316	0.279929790873122\\
321	0.234084847477705\\
326	0.226106861735771\\
331	0.199794897525405\\
336	0.184252274620771\\
341	0.190942868074714\\
346	0.189628114942043\\
351	0.192184323187728\\
356	0.195608518317235\\
361	0.218866176130508\\
366	0.245007098258538\\
371	0.2229435032551\\
376	0.166147435656592\\
381	0.12241530620082\\
386	0.121971170698951\\
391	0.142603371591545\\
396	0.151484876381117\\
401	0.154497778259015\\
406	0.159634798959504\\
411	0.14596010262818\\
416	0.128459358482897\\
421	0.12645534159124\\
426	0.129716632158882\\
431	0.120752986270853\\
436	0.167624373542372\\
441	0.231654803723816\\
446	0.241976200652652\\
451	0.254264440117836\\
456	0.264203472287137\\
461	0.267871459875092\\
466	0.222472683912032\\
471	0.169624436008447\\
476	0.159411721178595\\
481	0.165780837292696\\
486	0.188503207915857\\
491	0.193287671515615\\
496	0.154717482390913\\
501	0.122331477145051\\
506	0.11095862594254\\
511	0.106863217057229\\
516	0.112330814679439\\
521	0.114139023197719\\
526	0.136016520225247\\
531	0.155934722301169\\
536	0.157564780586164\\
541	0.166588703510838\\
546	0.195110293590159\\
551	0.23102753240248\\
556	0.205409305863715\\
561	0.159638655991088\\
566	0.122205722811673\\
571	0.0999145558571468\\
576	0.115753675078466\\
581	0.128144968744817\\
586	0.131456153769688\\
591	0.135500130621787\\
596	0.135364214948868\\
601	0.135202974095728\\
606	0.130921046192585\\
611	0.125710044569178\\
616	0.138232516087643\\
621	0.170368782499324\\
626	0.204944055965819\\
631	0.250090113416204\\
636	0.284413245688283\\
641	0.237069568075327\\
646	0.193831565306502\\
651	0.204272257223259\\
656	0.216821444064739\\
661	0.225357219169581\\
666	0.203793110031001\\
671	0.181497934438314\\
676	0.190948105772444\\
681	0.209204377499303\\
686	0.204911849265476\\
691	0.193645834262575\\
696	0.180237975034749\\
701	0.136139560751507\\
706	0.104562682829592\\
711	0.114283403560715\\
716	0.118502007909176\\
721	0.108885406698526\\
726	0.120382045433785\\
731	0.137930565143421\\
736	0.137017381988364\\
741	0.141119364093987\\
746	0.18860158664849\\
751	0.215957666598893\\
756	0.218938623944399\\
761	0.242799071997884\\
766	0.281304878538658\\
771	0.327690230412948\\
776	0.416417881930023\\
781	0.475008117319538\\
786	0.429617457269173\\
791	0.390434097954323\\
796	0.35290698369712\\
801	0.314755930496868\\
806	0.307701130300036\\
811	0.273734376528321\\
816	0.24800688020802\\
821	0.26018355480239\\
826	0.227362739970182\\
831	0.174469296475951\\
836	0.16941936229375\\
841	0.170774177690593\\
846	0.169893261260411\\
851	0.194883277644989\\
856	0.219509095298517\\
861	0.225893887074075\\
866	0.243298713603522\\
871	0.262903870757858\\
876	0.292050833015525\\
881	0.325762726496466\\
886	0.350683469426104\\
891	0.36488691322784\\
896	0.367041785046673\\
901	0.375794112434359\\
906	0.371924113789743\\
911	0.368969116534433\\
916	0.381638608038874\\
921	0.359249046506873\\
926	0.333014301426246\\
931	0.337683662058589\\
936	0.336511425046593\\
941	0.338835564754295\\
946	0.351181547807358\\
951	0.353942064831879\\
956	0.353869179476889\\
961	0.365165793978945\\
966	0.374820978748237\\
971	0.379448032525322\\
976	0.390244943007106\\
981	0.393331948500945\\
986	0.379802033275463\\
991	0.377670026786255\\
996	0.383047377376252\\
1001	0.370974619336124\\
1006	0.354205501821925\\
1011	0.354063857511817\\
1016	0.339869408061946\\
1021	0.308134554524247\\
1026	0.291570901009466\\
1031	0.27313953298018\\
1036	0.259335836988586\\
1041	0.257815249820446\\
1046	0.235047124957467\\
1051	0.216045083230334\\
1056	0.221538122034724\\
1061	0.21303901603958\\
1066	0.2012571261688\\
1071	0.217141093640618\\
1076	0.219361430483392\\
1081	0.209711585978921\\
1086	0.220092058262115\\
1091	0.220206789076909\\
1096	0.203543741669753\\
1101	0.207622398573636\\
1106	0.227672480024677\\
1111	0.22832102646098\\
1116	0.204787543980852\\
1121	0.188397693458642\\
1126	0.1925086799853\\
1131	0.183087260963659\\
1136	0.172321908845475\\
1141	0.183515333097839\\
1146	0.180418969023679\\
1151	0.166249495668333\\
1156	0.173749034364462\\
1161	0.185298940587318\\
1166	0.18007589882618\\
1171	0.183002170722685\\
1176	0.206987203939051\\
1181	0.206394211752834\\
1186	0.18402966452845\\
1191	0.174962949257657\\
1196	0.164479679745506\\
1201	0.15188481859352\\
1206	0.168919694299784\\
1211	0.194377931544641\\
1216	0.187217969347903\\
1221	0.167684957820899\\
1226	0.161336628690338\\
1231	0.16299217582502\\
1236	0.148996489485305\\
1241	0.139942968000542\\
1246	0.152718141008279\\
1251	0.164864942860367\\
1256	0.163422495818923\\
1261	0.150379973740197\\
1266	0.149489848441541\\
1271	0.154192390695427\\
1276	0.147154448392281\\
1281	0.146479523579335\\
1286	0.157016209317655\\
1291	0.168641439123411\\
1296	0.162624498085242\\
1301	0.151468227753927\\
1306	0.170862651901998\\
1311	0.193491629595987\\
1316	0.18956291792336\\
1321	0.197151913920163\\
1326	0.225691727486208\\
1331	0.225208060734277\\
1336	0.200381232605838\\
1341	0.19285416010983\\
1346	0.198995586464812\\
1351	0.185821185802035\\
1356	0.17596589499789\\
1361	0.207621152447919\\
1366	0.23952382073814\\
1371	0.222021143562404\\
1376	0.198748926877302\\
1381	0.199560673153177\\
1386	0.205994123321708\\
1391	0.20934067317491\\
1396	0.185971684644834\\
1401	0.177325399310473\\
1406	0.201211592012392\\
1411	0.207620132669928\\
1416	0.19239910681652\\
1421	0.187132986906229\\
1426	0.190180840149005\\
1431	0.16632959923245\\
1436	0.142352308482585\\
1441	0.155451019160519\\
1446	0.170217829884379\\
1451	0.153408590359379\\
1456	0.137866710213405\\
1461	0.137054235451397\\
1466	0.136116417466153\\
1471	0.127176962383119\\
1476	0.10592234096601\\
1481	0.099134298133995\\
1486	0.107882894224719\\
1491	0.120366546217562\\
1496	0.118753083378585\\
1501	0.109326516218965\\
1506	0.114736362115004\\
1511	0.110532779614594\\
1516	0.0991907890551304\\
1521	0.109925853100373\\
1526	0.123706992687735\\
1531	0.115113560124521\\
1536	0.111539134974866\\
1541	0.114741065520452\\
1546	0.11758973546384\\
1551	0.117637446996285\\
1556	0.110739732490824\\
1561	0.119374978257852\\
1566	0.139651326277486\\
1571	0.139264813865314\\
1576	0.132122640684374\\
1581	0.134419836489175\\
1586	0.130894702423858\\
1591	0.11773971464719\\
1596	0.104101367282225\\
1601	0.0983841956815089\\
1606	0.106265990422952\\
1611	0.117414588708354\\
1616	0.098453475694293\\
1621	0.0809146998259211\\
1626	0.0848000565183555\\
1631	0.0847246668474698\\
1636	0.0945272100181162\\
1641	0.0964542918238283\\
1646	0.0873105083739588\\
1651	0.0932764186302239\\
1656	0.0994543519435351\\
1661	0.0969107813526761\\
1666	0.0974294938989941\\
1671	0.102094091298306\\
1676	0.103458623914899\\
1681	0.103157393720774\\
1686	0.102631578913466\\
1691	0.100955143777884\\
1696	0.107287153201908\\
1701	0.120112730095176\\
1706	0.117857631568623\\
1711	0.115115423642369\\
1716	0.123632916326636\\
1721	0.132905938311212\\
1726	0.145668319159982\\
1731	0.133769007065993\\
1736	0.110801446218162\\
1741	0.111488865652273\\
1746	0.116468492055311\\
1751	0.110192813729452\\
1756	0.102211996526687\\
1761	0.101219289039535\\
1766	0.103977122665258\\
1771	0.0999489934973566\\
1776	0.0817881793073733\\
1781	0.0750996937025937\\
1786	0.105870485126471\\
1791	0.135760043277301\\
1796	0.133250630029392\\
1801	0.131777529454245\\
1806	0.137000037703856\\
1811	0.148117494993158\\
1816	0.163535946260201\\
1821	0.15513744193332\\
1826	0.133279894321234\\
1831	0.139661870341416\\
1836	0.164167448162222\\
1841	0.171929368710719\\
1846	0.160836520558081\\
1851	0.152406893365655\\
1856	0.15726880996261\\
1861	0.164499023997735\\
1866	0.167474557188766\\
1871	0.162332540985263\\
1876	0.158946973757406\\
1881	0.160445194975381\\
1886	0.16039722272891\\
1891	0.166359365682151\\
1896	0.159460622148835\\
1901	0.142189916639531\\
1906	0.138986426445637\\
1911	0.135351362880882\\
1916	0.129004927511192\\
1921	0.146334044362351\\
1926	0.172770044802829\\
1931	0.170496173723096\\
1936	0.152345009655297\\
1941	0.147096482458325\\
1946	0.151373865215459\\
1951	0.167775419535135\\
1956	0.182166414070377\\
1961	0.178617288704412\\
1966	0.174647059452936\\
1971	0.172789843962138\\
1976	0.155208271868224\\
1981	0.139367290792852\\
1986	0.134770994130856\\
1991	0.131291616025132\\
1996	0.129020660290555\\
2001	0.123797948091742\\
2006	0.11778344062462\\
2011	0.119288263014969\\
2016	0.12960381997901\\
2021	0.130457903649836\\
2026	0.117920409787729\\
2031	0.10906590972523\\
2036	0.109900053437816\\
2041	0.109607789134931\\
2046	0.100678080789444\\
2051	0.0823673427244661\\
2056	0.0821187475481483\\
2061	0.0956583492264801\\
2066	0.107264398474328\\
2071	0.124131788115449\\
2076	0.130794764459723\\
2081	0.12475280489792\\
2086	0.125500724431845\\
2091	0.123032907456533\\
2096	0.115923478134441\\
2101	0.124553816911486\\
2106	0.137388244487505\\
2111	0.140572701847127\\
2116	0.136996095888627\\
2121	0.134444976761152\\
2126	0.136043976065934\\
2131	0.141455514813174\\
2136	0.152410755964326\\
2141	0.163755318315588\\
2146	0.172476749748911\\
2151	0.17909073028833\\
2156	0.171564706135515\\
2161	0.162951739880293\\
2166	0.159778480979888\\
2171	0.152538017891893\\
2176	0.150623141653903\\
2181	0.155658734164818\\
2186	0.160728659071257\\
2191	0.163204035952066\\
2196	0.162899799679284\\
2201	0.153010742231962\\
2206	0.148362128390344\\
2211	0.155148972618932\\
2216	0.16031977749152\\
2221	0.155729236723295\\
2226	0.155025735757278\\
2231	0.15790376044339\\
2236	0.159636125318775\\
2241	0.162931430340488\\
2246	0.164067687723271\\
2251	0.155965953931632\\
2256	0.136579510688169\\
2261	0.127169864344277\\
2266	0.12991808158284\\
2271	0.129623896747314\\
2276	0.125064318794413\\
2281	0.135040676268602\\
2286	0.151175098772871\\
2291	0.147735204809098\\
2296	0.130273818854028\\
2301	0.121639158145856\\
2306	0.122536151637299\\
2311	0.121744087395376\\
2316	0.124870540420612\\
2321	0.126997019347122\\
2326	0.130051625867602\\
2331	0.13781357013288\\
2336	0.140191024293461\\
2341	0.139678882439893\\
2346	0.126656271376849\\
2351	0.109715648519552\\
2356	0.104251134541588\\
2361	0.109501046451003\\
2366	0.116284157203161\\
2371	0.116609272311595\\
2376	0.134491593181136\\
2381	0.152473194681638\\
2386	0.150372547698124\\
2391	0.148948535587487\\
2396	0.147635558743902\\
2401	0.145603314425971\\
2406	0.148977340359902\\
2411	0.152668589990761\\
2416	0.155672750420042\\
2421	0.159459875821497\\
2426	0.163173501117708\\
2431	0.156708434994949\\
2436	0.139701448063514\\
2441	0.127081566209843\\
2446	0.117375590947565\\
2451	0.116998701850852\\
2456	0.118525475057732\\
2461	0.127508815917554\\
2466	0.146813713926419\\
2471	0.142178270115556\\
2476	0.12573169284851\\
2481	0.120247057186473\\
2486	0.119409943491164\\
2491	0.121813767467432\\
2496	0.136329465886439\\
2501	0.14371997966896\\
2506	0.14461177096025\\
2511	0.151537554535479\\
2516	0.152205446261886\\
2521	0.15395898619969\\
2526	0.15015003708105\\
2531	0.142432503480034\\
2536	0.141427810058339\\
2541	0.146639382149399\\
2546	0.146638719433881\\
2551	0.151927042886408\\
2556	0.169686839891621\\
2561	0.174015712058013\\
2566	0.172651321695057\\
2571	0.17448580526619\\
2576	0.175112042107108\\
2581	0.183357575084187\\
2586	0.197491425271979\\
2591	0.203825767237088\\
2596	0.202422490953575\\
2601	0.198025816301286\\
2606	0.202984149970573\\
2611	0.206155339647369\\
2616	0.20095705857555\\
2621	0.200102016389093\\
2626	0.208111883144711\\
2631	0.217611819391698\\
2636	0.218834130985786\\
2641	0.236864325646056\\
2646	0.259373008078779\\
2651	0.260660850948804\\
2656	0.253271002991024\\
2661	0.248037920935726\\
2666	0.245114554232295\\
2671	0.244009274832853\\
2676	0.250680860801958\\
2681	0.252801411183145\\
2686	0.253339908476674\\
2691	0.259635928350266\\
2696	0.268234731432769\\
2701	0.272195008403927\\
2706	0.267487909045292\\
2711	0.264602124433215\\
2716	0.269509489562153\\
2721	0.26722057421184\\
2726	0.253824448738519\\
2731	0.257205659790384\\
2736	0.271665055177527\\
2741	0.284749873665136\\
2746	0.282827941293801\\
2751	0.266151280083715\\
2756	0.255358675255432\\
2761	0.263877815101282\\
2766	0.275334667856803\\
2771	0.273988602129444\\
2776	0.272446900993454\\
2781	0.282597668779925\\
2786	0.303589248117901\\
2791	0.313820877574023\\
2796	0.312697975105202\\
2801	0.308600440898362\\
2806	0.301797555080854\\
2811	0.29379431152441\\
2816	0.297573862079589\\
2821	0.315001805087529\\
2826	0.315918786829278\\
2831	0.295093958645457\\
2836	0.282053367831204\\
2841	0.278190788281844\\
2846	0.273513957557273\\
2851	0.275609995204046\\
2856	0.274402171990949\\
2861	0.272304749004979\\
2866	0.276740193616581\\
2871	0.28454741147056\\
2876	0.287012027473947\\
2881	0.280799540969231\\
2886	0.278222579305357\\
2891	0.277359815818901\\
2896	0.274398845006118\\
2901	0.274732790955549\\
2906	0.288665993165576\\
2911	0.305113503700747\\
2916	0.305347403245793\\
2921	0.301926470857273\\
2926	0.297054830149705\\
2931	0.287819235784898\\
2936	0.281595252323374\\
2941	0.273565503166308\\
2946	0.266856132282301\\
2951	0.265755035790073\\
2956	0.27115747193807\\
2961	0.272909727849562\\
2966	0.267362269384429\\
2971	0.264434156245919\\
2976	0.282301793413199\\
2981	0.314988156159359\\
2986	0.332830387493961\\
2991	0.346468812948908\\
2996	0.367351834579433\\
3001	0.390974489019571\\
3006	0.40366249953399\\
3011	0.398384560923926\\
3016	0.389930718049599\\
3021	0.40549866379033\\
3026	0.435355767852116\\
3031	0.450785139832121\\
3036	0.464185876055191\\
3041	0.497592980641374\\
3046	0.520145698430325\\
3051	0.517123176066905\\
3056	0.517375365353655\\
3061	0.509848244244359\\
3066	0.465252475361163\\
3071	0.414960881696426\\
3076	0.400409555221132\\
3081	0.402850745524456\\
3086	0.380275109066774\\
3091	0.327533385960924\\
3096	0.291671561005256\\
3101	0.26940701790226\\
3106	0.249105972355503\\
3111	0.232407648500748\\
3116	0.208584591734549\\
3121	0.186807652374176\\
3126	0.175133768564795\\
3131	0.175407630943974\\
3136	0.183429528293366\\
3141	0.186909101260254\\
3146	0.204553811693526\\
3151	0.261669700269462\\
3156	0.311323769366632\\
3161	0.32986145852851\\
3166	0.347573269844509\\
3171	0.383482368726699\\
3176	0.412975224450905\\
3181	0.417991577798513\\
3186	0.411595921642007\\
3191	0.399397262135176\\
3196	0.414170417139662\\
3201	0.447724384030685\\
3206	0.464027820949538\\
3211	0.465170873949384\\
3216	0.464492313203296\\
3221	0.464039037892984\\
3226	0.465111433001949\\
3231	0.468323144809158\\
3236	0.472507671025875\\
3241	0.47365689834107\\
3246	0.471840685333285\\
3251	0.480392137793654\\
3256	0.494146986934983\\
3261	0.49965050298567\\
3266	0.495871065989684\\
3271	0.486949277147194\\
3276	0.481950313876359\\
3281	0.48690399804005\\
3286	0.495488725130639\\
3291	0.491961587775448\\
3296	0.490691923507914\\
3301	0.500407450472864\\
3306	0.498232918793904\\
3311	0.481087327187627\\
3316	0.467294459231324\\
3321	0.460819901120826\\
3326	0.415237916074125\\
3331	0.355418479332551\\
3336	0.335210895982739\\
3341	0.334847503540985\\
3346	0.333993404753285\\
3351	0.310470450995992\\
3356	0.284552579725973\\
3361	0.279461084137756\\
3366	0.281535784693767\\
3371	0.295990819159139\\
3376	0.315232371604049\\
3381	0.329885281929965\\
3386	0.336451836595479\\
3391	0.354666499257795\\
3396	0.381554567214019\\
3401	0.390397366122539\\
3406	0.399955718992335\\
3411	0.430031930514364\\
3416	0.46035031011564\\
3421	0.478661477352606\\
3426	0.537635778123004\\
3431	0.594821388241266\\
3436	0.602752619477784\\
3441	0.599481006757286\\
3446	0.655435307823681\\
3451	0.72394655117949\\
3456	0.725778433704824\\
3461	0.716431302882096\\
3466	0.712229542945524\\
3471	0.702584078043112\\
3476	0.692531315465139\\
3481	0.685748572197401\\
3486	0.729252581882301\\
3491	0.780033095539925\\
3496	0.786999223096349\\
3501	0.790701509792855\\
3506	0.819461549023126\\
3511	0.854067179942098\\
3516	0.854848812935351\\
3521	0.843964716497064\\
3526	0.811480390379197\\
3531	0.767146529796949\\
3536	0.741238654906886\\
3541	0.730020975370291\\
3546	0.727078761126636\\
3551	0.7266056471346\\
3556	0.726510244726565\\
3561	0.725825021149427\\
3566	0.719552070811213\\
3571	0.735795935383535\\
3576	0.752172775017505\\
3581	0.744874615775894\\
3586	0.754999473648742\\
};

==> figures/setup.tex <==
%% Creator: Inkscape inkscape 0.92.5, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'setup.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{370.9873662bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.34824765)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0.03849173,0.11371815){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Plant $\mathbb{T}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{figures/setup.pdf}}%
    \put(0.2780689724,0.290342897){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Sensor $\mathbb{S}_1$\end{tabular}}}}%
    \put(0.278689724,0.0303625){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Sensor $\mathbb{S}_m$\end{tabular}}}}%
    \put(0.278689724,0.15258282){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Sensor $\mathbb{S}_2$\end{tabular}}}}%
    \put(0.5008165402,0.11371815){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Aggregator $\mathbb{A}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{figures/setup.pdf}}%
    \put(0.78273849,0.11371815){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Query Node $\mathbb{Q}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{figures/setup.pdf}}%
    \put(0.35091926,0.11371815){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}.\\.\\.\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{figures/setup.pdf}}%
    \put(0.77540737,0.30257248){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{2.25}\smash{\begin{tabular}[t]{l}not encrypted\end{tabular}}}}%
    \put(0.775059,0.27053949){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{2.25}\smash{\begin{tabular}[t]{l}encrypted\end{tabular}}}}%
    \put(0.77680005,0.23955106){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{2.25}\smash{\begin{tabular}[t]{l}coalition\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{figures/setup.pdf}}%
  \end{picture}%
\endgroup%


==> figures/setupGrp.tex <==
%% Creator: Inkscape inkscape 0.92.5, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'setupGrp.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{452.68382155bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.4342558)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0.03687046,0.20744846){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Plant $\mathbb{T}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{figures/setupGrp.pdf}}%
    \put(0.209550547,0.38526038){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\!Sensor $\mathbb{S}_1^{(1)}$\end{tabular}}}}%
    \put(0.209550547,0.28735932){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\!Sensor $\mathbb{S}_{m_1}^{(1)}$\end{tabular}}}}%
    \put(0.585259726,0.2123602){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Aggregator $\mathbb{A}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{figures/setupGrp.pdf}}%
    \put(0.820597171,0.21071615){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Query Node $\mathbb{Q}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{figures/setupGrp.pdf}}%
    \put(0.26610648,0.35233139){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}.\\.\\.\end{tabular}}}}%
    \put(0.383974178,0.33628954){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Manager $\mathbb{M}^{(1)}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{figures/setupGrp.pdf}}%
    \put(0.26548577,0.10802181){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}.\\.\\.\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{figures/setupGrp.pdf}}%
    \put(0.3505052799,0.40291979){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Sensor Group $\mathbb{G}^{(1)}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=6]{figures/setupGrp.pdf}}%
    \put(0.209550547,0.1427873){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\!Sensor $\mathbb{S}_1^{(d)}$\end{tabular}}}}%
    \put(0.209550547,0.04688621){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\!Sensor $\mathbb{S}_{m_d}^{(d)}$\end{tabular}}}}%
    \put(0.383974178,0.09381645){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Manager $\mathbb{M}^{(d)}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=7]{figures/setupGrp.pdf}}%
    \put(0.3505052799,0.00831839){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}Sensor Group $\mathbb{G}^{(d)}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=8]{figures/setupGrp.pdf}}%
    \put(0.36489295,0.22823191){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{0.25}\smash{\begin{tabular}[t]{l}.\\.\\.\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=9]{figures/setupGrp.pdf}}%
    \put(0.82893403,0.40223156){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{2.25}\smash{\begin{tabular}[t]{l}not encrypted\end{tabular}}}}%
    \put(0.82893403,0.37501295){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{2.25}\smash{\begin{tabular}[t]{l}encrypted\end{tabular}}}}%
    \put(0.82893403,0.34782295){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{2.25}\smash{\begin{tabular}[t]{l}coalition\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> figures/setuptex.tex <==
	\begin{figure*}[t]
	\centering
		\begin{tikzpicture}[scale=0.5, transform shape,line width=1pt]
		\draw (-3,0)  node[rectangle,draw,scale=1.5,line width=1pt] (plant)   {Plant $\mathbb{T}$};
		\draw (3,3)  node[rectangle,draw,scale=1.5,line width=1pt] (sensor1)   {Sensor $\mathbb{S}_1$};
		\draw (3,0)  node[rectangle,draw,scale=1.5,line width=1pt] (sensor12)   {Sensor $\mathbb{S}_i$};
		\draw (3,-3)  node[rectangle,draw,scale=1.5,line width=1pt] (sensorN)   {Sensor $\mathbb{S}_{m_a}$};
		\draw (9,0)  node[rectangle,draw,scale=1.5,line width=1pt] (cloud)   {Cloud $\mathbb{A}$};
				\draw (14,0)  node[rectangle,draw,scale=1.5,line width=1pt] (QN)   {Query Node $\mathbb{Q}$};
		\draw[->,dotted] (plant) -- (sensor1);
				\draw[->,dotted] (plant) -- (sensor12);
						\draw[->,dotted] (plant) -- (sensorN);
		\draw[->] (sensor1) -- (cloud);	
				\draw[->] (sensor12) -- (cloud);				
						\draw[->] (sensorN) -- (cloud);	
			\draw[<->] (cloud) -- (QN);								
		\end{tikzpicture}
	\caption{The systematic diagram where the dashed links are for sensing and the bold links are for information communication.}
	\label{fig:diagram}
\end{figure*}
